How I Learned to Stop Worrying and Love ChatGPT

In the dynamic landscape of software engineering, the emergence of ChatGPT-generated code signifies a distinctive and evolving paradigm in development practices. We delve into the impact of interactions with ChatGPT on the software development process, specifically analysing its influence on source code changes. Our emphasis lies in aligning code with ChatGPT conversations, separately analysing the user-provided context of the code and the extent to which the resulting code has been influenced by ChatGPT. Additionally, employing survival analysis techniques, we examine the longevity of ChatGPT-generated code segments in comparison to lines written traditionally. The goal is to provide valuable insights into the transformative role of ChatGPT in software development, illuminating its implications for code evolution and sustainability within the ecosystem.

==> conversations_table.tex <==
\setcounter{table}{0}
\begin{table}
\caption{Characteristics of ChatGPT conversations and associated  code changes}
\begin{tabular}{lrrrrll}
        \toprule
        ~ & ~ & ~ & \multicolumn{4}{l}{Median 95\% CI [low, high]}\\
    % ~ & ~ & ~ & l}{Conversations} & \multicolumn{2}{l}{Prompts/Answers} & \multicolumn{2}{l}{Prompt Tokens} & \multicolumn{2}{l}{Answer Tokens} \\
    Sharing type & Commits & Excluded & Conversations & Prompts & Prompt tok. & Answer tok. \\
            \midrule
    Pull Request & 182 & 4 & [1, 2] & [2, 2] & [92.5, 236] & [431, 599.5] \\
    Commit       & 691 & 5 & [1, 1] & [1, 1] & [676,  733] & [483, 557] \\
    Issue        & 69  & 0 & [1, 2] & [2, 3] & [92,   264] & [461, 757] \\
            \bottomrule
\end{tabular}
\end{table}


==> repositories_table.tex <==
\setcounter{table}{1}
\begin{table}
\caption{\centering Characteristics of the Software Repository}
    \begin{tabular}{lrrrrrr}
            \toprule
        ~ & ~ & \multicolumn{4}{l}{Median 95\% CI [low, high]}\\
        Sharing type & Repositories & Commits & Authors & Forks & Stars \\
             \midrule
        Pull Request & 210 & [407    , 736  ]& [14 , 25]& [12 , 37]& [22  , 91]\\
        Commit       & 76  & [37     , 95.52]& [1  , 3]& [0  , 0]& [0   , 1]\\ 
        Issue        & 382 & [147.45 , 244.5]& [5  , 7]& [2  , 5]& [6.5 , 21.5]\\ 
                \bottomrule
    \end{tabular}
\end{table}

